Neural Storage: A New Paradigm of Elastic Memory

Storage and retrieval of data in a computer memory plays a major role in system performance. Traditionally, computer memory organization is static - i.e., they do not change based on the application-specific characteristics in memory access behaviour during system operation. Specifically, the association of a data block with a search pattern (or cues) as well as the granularity of a stored data do not evolve. Such a static nature of computer memory, we observe, not only limits the amount of data we can store in a given physical storage, but it also misses the opportunity for dramatic performance improvement in various applications. On the contrary, human memory is characterized by seemingly infinite plasticity in storing and retrieving data - as well as dynamically creating/updating the associations between data and corresponding cues. In this paper, we introduce Neural Storage (NS), a brain-inspired learning memory paradigm that organizes the memory as a flexible neural memory network. In NS, the network structure, strength of associations, and granularity of the data adjust continuously during system operation, providing unprecedented plasticity and performance benefits. We present the associated storage/retrieval/retention algorithms in NS, which integrate a formalized learning process. Using a full-blown operational model, we demonstrate that NS achieves an order of magnitude improvement in memory access performance for two representative applications when compared to traditional content-based memory.

==> bibItemFile.tex <==
\begin{thebibliography}{}
\bibitem{ref:al2018survey } A. Al-Kaff,  D. Martin, F. Garcia, A. de la Escalera, and J.M. Armingol, ``Survey of computer vision algorithms and applications for unmanned aerial vehicles," Expert Systems with Applications, 2018.
\bibitem{ref:firedrone} {\'A} Rest{\'a}s, ``Thematic division and tactical analysis of the UAS application supporting forest fire management," Viegas, X.D., Ed., Advances in Forest Fire Research, 2014.
\bibitem{ref:koch2015review} C.~Koch, K.~Georgieva, K.~Kristina, A.~Varun, B.~Akinci, P.~Fieguth, ``A review on computer vision based defect detection and condition assessment of concrete and asphalt civil infrastructure," Advanced Engineering Informatics, 2015.
\bibitem{EESurvey} AspenCore, ``2019 embedded markets study," \url{https://www.embedded.com/wp-content/uploads/2019/11/EETimes_Embedded_2019_Embedded_Markets_Study.pdf}, 2019
\bibitem{azar2019energy}  Joseph~Azar, Abdallah~Makhoul, Mahmoud~Barhamgi, Rapha{\"e}l~Couturier,``An energy efficient IoT data compression approach for edge machine learning,"Future Generation Computer Systems,2019
\bibitem{AiIoT1000}  John~Koetsier,``AI + IoT = 1000X More Dense Networking Environments: How Intel, NSF Are Planning For Tomorrow,"\url{https://www.forbes.com/sites/johnkoetsier/2020/07/11/ai--iot--1000x-more-dense-networking-environments-how-intel-nsf-are-planning-for-tomorrow},2020
\bibitem{iotSpectrumSurvey} L.~{Z}hang,``Spectrum Sharing for Internet of Things: A Survey,"IEEE Wireless Communications,2019
\bibitem{ref:jpeg}  William B~Pennebaker, Joan L~Mitchell,``JPEG: Still image data compression standard,",1992
\bibitem{ref:webp} Google~,``WebP,"\url{https://developers.google.com/speed/webp}
\bibitem{ref:fireDS} Dataturks~,``ForestFire,"\url{https://dataturks.com/projects/qdyzl1013/Forest\%20Fire}
\bibitem{ref:crackDS} {\"O}~,``Performance comparison of pretrained convolutional neural networks on crack detection in buildings,"ISARC. Proceedings of the International Symposium on Automation and Robotics in Construction,2018
\bibitem{iotFaceDetection}  Ilhan~Aydin, Nashwan Adnan~Othman,``A new IoT combined face detection of people by using computer vision for security application,"2017 International Artificial Intelligence and Data Processing Symposium (IDAP),2017
\bibitem{arialFireDetection}  Chi~Yuan, Zhixiang~Liu, Youmin~Zhang,``Aerial images-based forest fire detection for firefighting using optical remote sensing techniques and unmanned aerial vehicles,"Journal of Intelligent \& Robotic Systems,2017
\bibitem{UAVRoofHole_IoT}  Shaodan~Li, Hong~Tang, Shi~He, Yang~Shu, Ting~Mao, Jing~Li, Zhihua~Xu,``Unsupervised detection of earthquake-triggered roof-holes from UAV images using joint color and shape features,"IEEE Geoscience and Remote Sensing Letters,2015
\bibitem{UAV_earthquake_IoT}  D~Duarte, F~Nex, N~Kerle, G~Vosselman,``Towards a more efficient detection of earthquake induced facade damages using oblique UAV imagery,"The International Archives of Photogrammetry, Remote Sensing and Spatial Information Sciences,2017
\bibitem{floodIoT}  Bilal~Arshad, Robert~Ogie, Johan~Barthelemy, Biswajeet~Pradhan, Nicolas~Verstaevel, Pascal~Perez,``Computer Vision and IoT-Based Sensors in Flood Monitoring and Mapping: A Systematic Review,"Sensors,2019
\bibitem{sadler2006data}  Christopher M~Sadler, Margaret~Martonosi,``Data compression algorithms for energy-constrained devices in delay tolerant networks,"Proceedings of the 4th international conference on Embedded networked sensor systems,2006
\bibitem{ref:deepnjpeg}  Zihao~Liu, Tao~Liu, Wujie~Wen, Lei~Jiang, Jie~Xu, Yanzhi~Wang, Gang~Quan,``DeepN-JPEG: a deep neural network favorable JPEG-based image compression framework,"Proceedings of the 55th Annual Design Automation Conference,2018
\bibitem{ref:weber2019lossy}  Maurice~Weber, Cedric~Renggli, Helmut~Grabner, Ce~Zhang,``Lossy Image Compression with Recurrent Neural Networks: from Human Perceived Visual Quality to Classification Accuracy,"arXiv preprint arXiv:1910.03472,2019
\bibitem{ref:marwood2018representing}  David~Marwood, Pascal~Massimino, Michele~Covell, Shumeet~Baluja,``Representing images in 200 bytes: Compression via triangulation,"IEEE International Conference on Image Processing,2018
\bibitem{arithmeticCoding_1}  Roger J~Clarke,``Digital compression of still images and video,",1995
\bibitem{arithmeticCoding_2}  Glen G~Langdon,``An introduction to arithmetic coding,"IBM Journal of Research and Development,1984
\bibitem{huffman} D.~A.,``A Method for the Construction of Minimum-Redundancy Codes,"Proceedings of the IRE,1952
\bibitem{imageCompSurvey}  Abir Jaafar~Hussain, Ali~Al-Fayadh, Naeem~Radi,``Image compression techniques: A survey in lossless and lossy algorithms,"Neurocomputing,2018
\bibitem{ref:rippel2017real}  Oren~Rippel, Lubomir~Bourdev,``Real-time adaptive image compression,"Proceedings of the 34th International Conference on Machine Learning-Volume 70,2017
\bibitem{ref:toderici2017full}  George~Toderici, Damien~Vincent, Nick~Johnston, Sung~Jin Hwang, David~Minnen, Joel~Shor, Michele~Covell,``Full resolution image compression with recurrent neural networks,"Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition,2017
\bibitem{ref:Li_2018_CVPR}  Mu~Li, Wangmeng~Zuo, Shuhang~Gu, Debin~Zhao, David~Zhang,``Learning Convolutional Networks for Content-Weighted Image Compression,"The IEEE Conference on Computer Vision and Pattern Recognition,2018
\bibitem{ref:balle2018variational} Ball{\'e}~,``Variational image compression with a scale hyperprior,"arXiv preprint arXiv:1802.01436,2018
\bibitem{ref:medical}  Zihao~Liu, Xiaowei~Xu, Tao~Liu, Qi~Liu, Yanzhi~Wang, Yiyu~Shi, Wujie~Wen, Meiping~Huang, Haiyun~Yuan, Jian~Zhuang,``Machine vision guided 3d medical image compression for efficient transmission and accurate segmentation in the clouds,"Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition,2019
\bibitem{scikit-learn}  F.~Pedregosa, G.~Varoquaux, A.~Gramfort, V.
        ~Michel, B.~Thirion, O.~Grisel, M.~Blondel, P.
        ~Prettenhofer, R.~Weiss, V.~Dubourg, J.~Vanderplas, A. and
         Cournapeau~Passos, M.~Brucher, M.~Perrot, E.~Duchesnay,``Scikit-learn: Machine Learning in {P,"Journal of Machine Learning Research,2011}
\bibitem{chollet2015keras}  Fran\c{c}~Chollet,``Keras,"\url{https://keras.io,2015}
\bibitem{scikit-image}  {S}~van der Walt,``scikit-image: image processing in {P,"PeerJ},2014
\bibitem{imagemagick} {The~ImageMagick,``ImageMagick,"},
\bibitem{ref:vgg}  Karen~Simonyan, Andrew~Zisserman,``Very deep convolutional networks for large-scale image recognition,"arXiv preprint arXiv:1409.1556,2014

% \bibitem{azar2019energy}
\end{thebibliography}

==> equations/contentBasedFetch.tex <==
Assume $M =$ Set of Data and Cue in the Memory at a given instance. To fetch a data $D \in M$, the query must consist of a reference data ${D}$' such that ${D}' \approx D$.

==> equations/impreciseStoreRet.tex <==
Assume $M =$ Set of Data and Cue in the Memory at a given instance. For a data $D \in M$, if $D$ is compressed (by lossy paradigm) to ${D}'$ then: 
\\ \hspace*{1mm} $(size(D) = size({D}') - \epsilon_1)  \implies$ 
\\ \hspace*{1mm} $(Usefulness ({D}') \neq 0) \land$
\\ \hspace*{1mm} $(Usefulness ({D}') = Usefulness ({D}') - \epsilon_2)$,
\\
Where size(X) is the size of the data X and Usefulness(X) is the quality indicator of the data X, in light of the specific application.

==> equations/ooi.tex <==
Assume that D is a new incoming data which must be stored in the Memory. Assume that, $LL = $Set of localities in the Memory Hive. $OL = $Objects in data D. $LO(L) = $Object class set assigned to locality L. $Class(O) = $Object class of O. $P(L) = $Priority of Locality $L$. Then the new data D is assigned to Locality $L_1$ if $\exists O_1 \in OL$ such that:
\\ \hspace*{1mm} $Class(O_1) \in LO(L_1) \land$
\\ \hspace*{1mm} $\nexists O_2 \mid O_2 \in OL \land Class(O_2) \in LO(L_2) \land P(L_2) > P(L_1)$
This condition ensures that the new Data, D is assigned to the Locality with highest priority such that there is at least one object in the data belonging to that locality. 

==> fig_latex/MemoryRetention.tex <==
\begin{figure*}[h!]
\centering
\includegraphics[width=\textwidth]{fig/MemoryRetention.png}
\caption{BINGO operation for background memory retention operation.}
\label{fig:MemoryRetention}
\end{figure*}

==> fig_latex/UAVSurv_Car_Constrained.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=\columnwidth]{fig/UAVSurv_Car_Constrained.png}
\caption{Plot comparing the Quality Factor of Traditional CAM with BINGO-2 for UAV-based surveillance for safety application in memory constrained settings. Frames containing car(s) are prioritized.}
\label{fig:UAVSurv_Car_Constrained}
\end{figure}

==> fig_latex/UAVSurv_Car_FetchAccess.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=\columnwidth]{fig/UAVSurv_Car_FetchAccess.png}
\caption{Plots showing data fetch efficiency of different BINGO modes in comparison to Traditional CAM for UAV-based surveillance for safety application. Frames containing car(s) are prioritized.}
\label{fig:UAVSurv_Car_FetchAccess}
\end{figure}

==> fig_latex/UAVSurv_Car_MemSize.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=\columnwidth]{fig/UAVSurv_Car_MemSize.png}
\caption{Plot of memory space utilization for UAV-based surveillance for safety application. Frames containing car(s) are prioritized.}
\label{fig:UAVSurv_Car_MemSize}
\end{figure}

==> fig_latex/WildLifeDS_Deer_Constrained.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=\columnwidth]{fig/WildLifeDS_Deer_Constrained.png}
\caption{Plot comparing the Quality Factor of Traditional CAM with BINGO-2 for wildlife surveillance application in memory constrained settings. Frames containing deer are prioritized.}
\label{fig:WildLifeDS_Deer_Constrained}
\end{figure}

==> fig_latex/WildLifeDS_Deer_FetchAccess.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=\columnwidth]{fig/WildLifeDS_Deer_FetchAccess.png}
\caption{Plots showing data fetch efficiency of different BINGO modes in comparison to Traditional CAM for wildlife surveillance application. Frames containing deer are prioritized.}
\label{fig:WildLifeDS_Deer_FetchAccess}
\end{figure}

==> fig_latex/WildLifeDS_Deer_MemSize.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=\columnwidth]{fig/WildLifeDS_Deer_MemSize.png}
\caption{Plot of memory space utilization for wildlife surveillance application. Frames containing deer are prioritized.}
\label{fig:WildLifeDS_Deer_MemSize}
\end{figure}

==> fig_latex/WildLifeDS_Fox_Constrainted.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=\columnwidth]{fig/WildLifeDS_Fox_Constrainted.png}
\caption{Plot comparing the Quality Factor of Traditional CAM with BINGO-2 for for wildlife surveillance application in memory constrained settings. Frames containing fox/wolf are prioritized.}
\label{fig:WildLifeDS_Fox_Constrainted}
\end{figure}

==> fig_latex/WildLifeDS_Fox_FetchAccess.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=\columnwidth]{fig/WildLifeDS_Fox_FetchAccess.png}
\caption{Plots showing data fetch efficiency of different BINGO modes in comparison to Traditional CAM for wildlife surveillance application. Frames containing fox/wolf are prioritized.}
\label{fig:WildLifeDS_Fox_FetchAccess}
\end{figure}

==> fig_latex/WildLifeDS_Fox_MemSize.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=\columnwidth]{fig/WildLifeDS_Fox_MemSize.png}
\caption{Plot of memory space utilization for wildlife surveillance application. Frames containing fox/wolf are prioritized.}
\label{fig:WildLifeDS_Fox_MemSize}
\end{figure}

==> fig_latex/dataRet.tex <==
\begin{figure*}[h!]
\centering
\includegraphics[width=\textwidth]{fig/dataRet.png}
\caption{BINGO algorithm for Data Load/Read operation.}
\label{fig:dataRet}
\end{figure*}

==> fig_latex/dataStorage.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=\columnwidth]{fig/dataStorage.png}
\caption{BINGO algorithm for Data Store/Write Operation.}
\label{fig:dataStorage}
\end{figure}

==> fig_latex/dataUnit.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=\columnwidth]{fig/dataUnit.png}
\caption{dataUnit}
\label{fig:dataUnit}
\end{figure}

==> fig_latex/dataUnitStatMonitor.tex <==
\begin{figure*}[h!]
\centering
\includegraphics[width=\textwidth]{fig/dataUnitStatMonitor.png}
\caption{Plots showing Data Neuron size and memory strength evolution with time.}
\label{fig:dataUnitStatMonitor}
\end{figure*}

==> tables/BINGO_Car_Main.tex <==
\begin{table*}[]
\centering
\caption{Simulation results for UAV-based surveillance application with frames containing car(s) being prioritized. BINGO performs as well as traditional CAM in terms of PSNR and SSIM of retrieved images. Hence, application performance does not get hampered. At the same time, BINGO is utilizing much less space and mean operation cost is far lower in comparison to Standard/Traditional CAM.}
\label{BINGO_Car_Main}
\renewcommand{\arraystretch}{1}
\scriptsize\addtolength{\tabcolsep}{2pt}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{ECF4FF} 
\textbf{Mode}                            & \textbf{PSNR} & \textbf{SSIM} & \textbf{AVG Retrieval Op. Cost} & \textbf{AVG Store Op. Cost} & \textbf{Mean Op. Cost} & \textbf{Memory Size (MB)} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{Trad. CAM} & 30.57         & 0.71          & 1870.41                & 0                      & 935.205                     & 801.14                    \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{BINGO-0} & 32.45         & 0.79          & 34.01                  & 36.94                  & 35.475                      & 34.82                     \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{BINGO-1} & 32.39         & 0.78          & 11.19                  & 26.39                  & 18.79                       & 34.51                     \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{BINGO-2} & 32.42         & 0.78          & 6.03                   & 22.67                  & 14.35                       & 34.67                     \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{BINGO-3} & 32.39         & 0.78          & 11.19                  & 26.38                  & 18.785                      & 34.51                     \\ \hline
\end{tabular}
\end{table*}

==> tables/BINGO_Deer_Main.tex <==
\begin{table*}[]
\centering
\caption{Simulation results for wildlife surveillance application. Frames containing deer(s) are prioritized. Judging by the PSNR and SSIM of the retrieved images, it is clear that BINGO provides similar performance in terms of the quality of retrieved data with respect to Traditional(Trad.) CAM. At the same time, BINGO is utilizing much less space and mean operation cost is far lower in comparison to Standard/Traditional CAM.}
\label{BINGO_Deer_Main}
\renewcommand{\arraystretch}{1}
\scriptsize\addtolength{\tabcolsep}{2pt}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{ECF4FF} 
\textbf{Mode}                            & \textbf{PSNR} & \textbf{SSIM} & \textbf{AVG Retrieval Op. Cost} & \textbf{AVG Store Op. Cost} & \textbf{Mean Op. Cost} & \textbf{Memory Size (MB)} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{Trad. CAM} & 37.65         & 0.79          & 5573.93                & 0                      & 2786.965                    & 2688.79                   \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{BINGO-0} & 38.41         & 0.82          & 68.84                  & 81.81                  & 75.325                      & 89.50                     \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{BINGO-1} & 38.3          & 0.82          & 12.66                  & 33.06                  & 22.86                       & 89.35                     \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{BINGO-2} & 38.39         & 0.82          & 5.51                   & 28.23                  & 16.87                       & 89.46                     \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{BINGO-3} & 38.3          & 0.82          & 12.66                  & 32.71                  & 22.685                      & 89.35                     \\ \hline
\end{tabular}
\end{table*}

==> tables/BINGO_Fox_Main.tex <==
\begin{table*}[]
\centering
\caption{Simulation results for Wildlife Surveillance application with an emphasis on fox/wolf images. Similar trends as seen in Table.~\ref{BINGO_Deer_Main} are observed. The PSNR and SSIM of retrieved images for all BINGO modes and traditional CAM are similar. This leads us to believe that, the application performance will not be hampered for using BINGO. At the same time, BINGO is utilizing much less space and mean operation cost is far lower in comparison to Standard/Traditional CAM.}
\label{BINGO_Fox_Main}
\renewcommand{\arraystretch}{1}
\scriptsize\addtolength{\tabcolsep}{2pt}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{ECF4FF} 
\textbf{Mode}                            & \textbf{PSNR} & \textbf{SSIM} & \textbf{AVG Retrieval Op. Cost} & \textbf{AVG Store Op. Cost} & \textbf{Mean Op. Cost} & \textbf{Memory Size (MB)} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{Trad. CAM} & 37.11         & 0.75          & 3306.83                & 0                      & 1653.415                    & 2688.79                   \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{BINGO-0} & 38.65         & 0.79          & 19.5                   & 57.28                  & 38.39                       & 97.04                     \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{BINGO-1} & 39            & 0.83          & 6.87                   & 24.3                   & 15.585                      & 96.96                     \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{BINGO-2} & 38.52         & 0.79          & 4.39                   & 22.96                  & 13.675                      & 97.40                     \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{BINGO-3} & 39            & 0.83          & 6.87                   & 24.06                  & 15.465                      & 96.96                     \\ \hline
\end{tabular}
\end{table*}
